Kaolin: A PyTorch Library for Accelerating 3D Deep Learning Research

We present Kaolin, a PyTorch library aiming to accelerate 3D deep learning research. Kaolin provides efficient implementations of differentiable 3D modules for use in deep learning systems. With functionality to load and preprocess several popular 3D datasets, and native functions to manipulate meshes, pointclouds, signed distance functions, and voxel grids, Kaolin mitigates the need to write wasteful boilerplate code. Kaolin packages together several differentiable graphics modules including rendering, lighting, shading, and view warping. Kaolin also supports an array of loss functions and evaluation metrics for seamless evaluation and provides visualization functionality to render the 3D results. Importantly, we curate a comprehensive model zoo comprising many state-of-the-art 3D deep learning architectures, to serve as a starting point for future research endeavours. Kaolin is available as open-source software at https://github.com/NVIDIAGameWorks/kaolin/.

==> 03_applications.tex <==
\section{Applications}
\label{sec:applications}

Kaolin aims to provide a one-stop package for all 3D deep learning tasks, and as such provides out of the box support for a wide array of applications. This section will highlight a number of 3d learning methods, borken down by the representation they employ, which are easily implemented through Kaolin's support, and available directly through the package.
% For a full list of methods we support please refer to the appendix. 
% \ED{lets add a full list of models in an appendix}


\subsection{Meshes}

For the mesh representation we provide a large number of methods, over a few tasks. For the task of image to 3D object reconstruction with full 3D supervision our methods include a simple baseline, the Pixel2Mesh algorithm \cite{Pixel2Mesh}, and the GEOMetrics algorithm \cite{GEOMetrics} are provided. Each rely on extracting image features from a image using a CNN, to deform a pherical mesh to match a target image, through varying deformation schemes and losses. 

% The simple baseline method consist of a single deep CNN which is passed the conditioning image and output updates for the positions vertices over a predefined mesh. Pixel2Mesh imroves on this baseline through per-vertex sampling of image features, Graph convolutional networks(GCNs) for mesh deformation, and iterative mesh refinement. GEOMetrics extends Pixel2Mesh through adaptive mesh up-scaling, modifying the GCN definition, novel geometric-based loss functions. 

For the task of 3D object reconstruction with only 2D supervision we support Neural 3D Mesh Renderer~\cite{NMR}, Soft-Rasterizer~\cite{softras}, and DIB-Renderer~\cite{dib} which each rely on some realization of a differentiable renderer. NMR hand-designs an approximate gradient definition for face movement across pixels, and predicts only a silhouette. Soft-Rasterizer fuses the probabilistic contributions of all mesh triangles with respect to each rendered pixel to produce full colour images. DIB-Renderer allows gradients to be analytically computed for all pixels in an image by viewing foreground and background rasterization as a weighted interpolation of local properties and global geometry. 

For arbitrary learning over meshes, in addition to generic Graph Convolutional Networks, we also support the MeshCNN method \cite{meshcnn}, which proposes a new convolutional-style architecture specifically designed for 2-manifold triangle meshes. 


% \begin{figure}[!thb]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/human_seg.png}
%     \caption{MeshCNN \cite{meshcnn} segmenting a human body.}
%     \label{fig:human_seg}
% \end{figure}

\subsection{SDFs}

For the SDF representation, Occupancy Networks, Deep Implicit Surface Network, and DeepSDF methods are supported. In the Occupancy Networks algorithm~\cite{Occ}, a simple CNN encoder feeds image information into a ResNet with conditional Batch normalization to predict occupancy values of random points in a predefined grid. The Deep Implicit Surface Network method \cite{DISN}, predicts where a queried point is projected on computed local image features to directly regress signed distance values from a conditioning image. DeepSDF~\cite{deepsdf} learns distributions of 3D shape and represents their signed distance functions via latent code-conditioned feed-forward decoder networks. 


\subsection{Point Clouds}
Over point clouds we support two main methods; PointNet and PointNet++. PointNet proposes a permutation invariant network architecture that acts directly on point clouds.  This provides a unified architecture for applications across point clouds such as object classification, part segmentation, and scene semantic parsing. PointNet++ extends PointNet by iterative partitioning and clustering points through the network to grow a global point cloud understanding in a hierarchical manner. 

% \begin{figure}[!thb]
%     \centering
%     \includegraphics[width=0.5\textwidth]{figures/voxelgan_chairs.png}
%     \caption{A collection of chairs generated by 3D-IWGAN~\cite{3DIWGAN}.}
%     \label{fig:voxelgan_chairs}
% \end{figure}


\subsection{Voxels}

We support voxel generative modelling through the 3D-GAN~\cite{3DGAN} method and its extension 3D-IWGAN~\cite{3DIWGAN}. Both apply generative adversarial networks to producing generators for distributions of 3D shapes, though the first with the standard GAN loss and the section with the Wasserstein GAN. Two methods are provided for voxel 3D reconstruction methods from images. The first is 3D-R2N2, where given one or multiple images of an object, its 3D shape is reconstructed through the use of LSTMs modified for 3D settings. The second methods is multi-view decomposition, which performs super-resolutions on extracted depth maps from a predicted 3D objects to produce high resolution 3D reconstructions. 

% \Krishna{Will add more viz in here as they come in.}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figures/applications2.png}
    \caption{\textbf{Applications of \kaolin{}}: }
    \label{fig:applications}
\end{figure*}



% \subsection{Differentiable renderers}


% \Krishna{Skeleton: Of late, there's this trend in 3D vision research of fusing known concepts from computer graphics (eg. shading, rendering, etc.) for unsupervised learning of 3D reconstruction. ... To make this nascent area of research accessible to a wider audience, as well as to enable researchers in the field push the area ahead, we contain a DR module. We design a modular DR abstract class, and show that existing DRs fall under this design. Specifically, we have 3 DRs: NMR, SoftRas, DIB-R. Major components of the DR are all abstractmethods that anyone implementing a new DR can override: Lighting/Shading/SceneSetup/Projection/Rasterization. (Lighting: Ambient, Directional, Specular), (Shading: Phong, Cosine), (Rasterization: NMR, SoftRas, DIB-R)}
% \TODO{ dont we already say all this? can we not remove this section?}

